Gravitational Wave Tests of General Relativity with Ground-Based Detectors and Pulsar Timing Arrays

This review is focused on tests of Einstein's theory of General Relativity with gravitational waves that are detectable by ground-based interferometers and pulsar timing experiments. Einstein's theory has been greatly constrained in the quasi-linear, quasi-stationary regime, where gravity is weak and velocities are small. Gravitational waves will allow us to probe a complimentary, yet previously unexplored regime: the non-linear and dynamical strong-field regime. Such a regime is, for example, applicable to compact binaries coalescing, where characteristic velocities can reach fifty percent the speed of light and compactnesses can reach a half. This review begins with the theoretical basis and the predicted gravitational wave observables of modified gravity theories. The review continues with a brief description of the detectors, including both gravitational wave interferometers and pulsar timing arrays, leading to a discussion of the data analysis formalism that is applicable for such tests. The review ends with a discussion of gravitational wave tests for compact binary systems.

==> cosmological-tests.tex <==
% Xavi write this
%
%   a-Polarization Tests
%   b-Primordial Black Holes and Quantum Gravity
%   c-Cosmic Strings and Phase Transitions
%------------------------------------------------------------------------------------------------------------------------------

%------------------------------------------------------------------------------------------------------------------------------
\subsection{Polarization tests}

{\bf{NY: You might want to mention here something like what's next. 
Most investigations of gravitational wave (GW) signatures of parity violation
have focused on {\emph{amplitude birefringence}}.
That is, compared to GR, right circularly-polarized waves are enhanced or suppressed and left circularly-polarized
waves are suppressed or enhanced as they propagate~\cite{Jackiw:2003pm,Lue:1998mq,Alexander:2007kv,Yunes:2008bu,Alexander:2009tp}.
Such birefringence occurs when GWs propagate on a flat or curved background. 
In fact, the propagation of such waves over cosmological distances has been proposed as an explanation 
of the baryogenesis problem in the early Universe~\cite{Alexander:2004us} and could have observable effects on
the cosmic microwave background~\cite{Alexander:2004wk, Saito:2007kt,
Contaldi:2008yz} and a stochastic GW background~\cite{Seto:2007tn,
Satoh:2007gn}.}}

%------------------------------------------------------------------------------------------------------------------------------
\subsection{Primordial black holes and quantum gravity}

%------------------------------------------------------------------------------------------------------------------------------
\subsection{Cosmic strings and phase transitions}


==> pulsar-tests.tex <==
% Nico and Xavi write this
%
%   a-Polarization Tests
%   b-Propagation tests (massive graviton)	
%------------------------------------------------------------------------------------------------------------------------------

{\comment{NY: One might wish to discuss somewhere in this section that spontaneous scalarization could lead to strong modifications to GW signals emitted by ``mountains'' on neutron stars. These modifications, however, will be degenerate with the equation of state, so it is unclear how well they can be constrained. On a similar note, Damour and company suggested that binary pulsar observations~\cite{Damour:1996ke,Damour:1998jk,Sotani:2004rq} could constrain this spontaneous scalarizations much better than GW observations. We might wish to discuss this in this section as well.}}

{\comment{NY: Remember to mention tests of the mass of the graviton with PTAs, from e.g. Lee, Jenet, Price, Wex and Kramer.}}

%------------------------------------------------------------------------------------------------------------------------------
\subsection{Polarization tests}

%------------------------------------------------------------------------------------------------------------------------------
\subsection{Propagation tests}



